Spatially relaxed inference on high-dimensional linear models

We consider the inference problem for high-dimensional linear models, when covariates have an underlying spatial organization reflected in their correlation. A typical example of such a setting is high-resolution imaging, in which neighboring pixels are usually very similar. Accurate point and confidence intervals estimation is not possible in this context with many more covariates than samples, furthermore with high correlation between covariates. This calls for a reformulation of the statistical inference problem, that takes into account the underlying spatial structure: if covariates are locally correlated, it is acceptable to detect them up to a given spatial uncertainty. We thus propose to rely on the $\delta$-FWER, that is the probability of making a false discovery at a distance greater than $\delta$ from any true positive. With this target measure in mind, we study the properties of ensembled clustered inference algorithms which combine three techniques: spatially constrained clustering, statistical inference, and ensembling to aggregate several clustered inference solutions. We show that ensembled clustered inference algorithms control the $\delta$-FWER under standard assumptions for $\delta$ equal to the largest cluster diameter. We complement the theoretical analysis with empirical results, demonstrating accurate $\delta$-FWER control and decent power achieved by such inference algorithms.

==> Makefile <==
LATEX=pdflatex -synctex=1
LATEXOPT=--shell-escape
NONSTOP=--interaction=nonstopmode

LATEXMK=latexmk
LATEXMKOPT=-pdf -view=none
CONTINUOUS=-pvc

MAIN=ecdl_proofs
SOURCES=$(MAIN).tex Makefile commands.tex extracted.bib
FIGURES := $(shell find prebuiltimages/* -type f)

all: once

watch: .refresh $(MAIN).pdf

.refresh:
	touch .refresh

$(MAIN).pdf: $(MAIN).tex .refresh $(SOURCES) $(FIGURES)
	$(LATEXMK) $(LATEXMKOPT) $(CONTINUOUS) \
		-pdflatex="$(LATEX) $(LATEXOPT) $(NONSTOP) %O %S" $(MAIN)

force:
	touch .refresh
	rm $(MAIN).pdf
	$(LATEXMK) $(LATEXMKOPT) $(CONTINUOUS) \
	    -pdflatex="$(LATEX) $(LATEXOPT) %O %S" $(MAIN)

clean:
	$(LATEXMK) -C $(MAIN)
	rm -f $(MAIN).pdfsync
	rm -rf *~ *.tmp
	rm -f *.bbl *.blg *.aux *.end *.fls *.log *.out *.brf *.fdb_latexmk *.synctex.gz *.synctex.gz\(busy\)

once:
	$(LATEXMK) $(LATEXMKOPT) -pdflatex="$(LATEX) $(LATEXOPT) %O %S" $(MAIN)

debug:
	$(LATEX) $(LATEXOPT) $(MAIN)

.PHONY: clean force once all watch

